Enhancing Creative Generation on Stable Diffusion-based Models

Recent text-to-image generative models, particularly Stable Diffusion and its distilled variants, have achieved impressive fidelity and strong text-image alignment. However, their creative capability remains constrained, as including `creative' in prompts seldom yields the desired results. This paper introduces C3 (Creative Concept Catalyst), a training-free approach designed to enhance creativity in Stable Diffusion-based models. C3 selectively amplifies features during the denoising process to foster more creative outputs. We offer practical guidelines for choosing amplification factors based on two main aspects of creativity. C3 is the first study to enhance creativity in diffusion models without extensive computational costs. We demonstrate its effectiveness across various Stable Diffusion-based models.

==> sec/5_discussion_fake.tex <==
\section{Discussions}
\label{sec:discussion}

\subsection{How C3 Enhances Creativity}

\textbf{``Creative'' Ablation.} We hypothesize that C3 only amplifies creativity when the prompt explicitly includes ``creative.'' Enlarging the latent boosts cross-attention values associated with the creative object, enhancing its generation. To verify this, we ablate the ``creative" in prompt and find that its removal results in ordinary images without noticeable artifacts (see Figure~\ref{fig:abl_creative}). The FID score even decreases, indicating that C3 does not generate unexpected images without ``creative" in prompt. 

% This is because enlarging the latent increases the cross-attention values associated with the creative object, enhancing its generation. To verify this, we ablate the ``creative" in prompt and find that its removal results in ordinary images with no noticeable artifacts (see Figure~\ref{fig:abl_creative}). The FID score even decreases, indicating that C3 does not generate unexpected images without ``creative" in prompt. 
\begin{figure}[h!]
  \centering
         \includegraphics[width=\columnwidth]{figure/ablate_creative_v3.pdf}
         \caption{(Left) Images generated with and without ``creative" in prompts.  (Right) Change in FID scores after applying C3.}
         \label{fig:abl_creative}  
\end{figure}

\noindent\textbf{Justification for C3.} 
To further support our hypothesis, we examine whether amplifying first-block features increases the second-block cross-attention map. 
% A one-sided t-test on mean attention values 
The \textit{t}-test results confirm a significant increase for the cross-attention map of ``[obj]"
% \footnote{[obj] implies creative [obj] due to the self-attention in text encoder.} 
in both Turbo and Lightning model with p-value $<e^{-30}$.
% The results confirm that C3 significantly enhances creativity-related object attention. 
% As shown in Table~\ref{table:t-test}, for both models, the cross-attention map for the ``[obj]"\footnote{[obj] implies creative [obj] due to the self-attention in text encoder.} token significantly increase. The results confirm that C3 significantly enhances creativity-related object attention. 
% While low-frequency features clearly enhance creativity in content, creativity driven by high-frequency features appears as colorful mosaics or noise (see Figure 4 in Sec. 3), requiring further investigation. We also automatically select the amplification factor based on the usability score to maintain generation quality.
C3 amplifies only low-frequency features which clearly enhance creativity in contents, as creativity driven by high-frequency features appears as colorful mosaics or noise (see Figure 4 in Sec. 3). We also automatically select the amplification factor based on the usability score to maintain generation quality.

% \noindent\textbf{Comparison with FreeU}
% C3 enhances creativity by selectively amplifying low-frequency backbone features with block-specific parameters, while FreeU~\cite{si2024freeu} attenuates low-frequency skip features ($s$) and boosts backbone features without frequency-based control ($b$), prioritizing fidelity. This distinction enables C3 to better steer creativity. In Figure~\ref{fig:freeu}, FreeU yields less clean and creative results than C3, regardless of parameters. Especially, for $b > 1$, noise persists irrespective of $s$.
% \begin{figure}[h!]
%   \centering
%          \includegraphics[width=\columnwidth]{figure/freeu-comparison-v2.pdf}
%          \vspace{-0.8cm}
%          \caption{Results with prompt  ``A creative chair'' in SDXL-Turbo.}
%          \label{fig:freeu}
  
% \end{figure}
% \subsection{Step-wise Analysis}

% \begin{figure}[!t]
%   \centering
%   %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  
%          \includegraphics[width=\columnwidth]{figure/step-analysis.pdf}
%          \caption{Step-wise amplification results on SDXL (step=50). Significant changes are observed in the earlier steps.  
%          }
%          \label{fig:step}
  
% \end{figure}
% Diffusion models operate through a multi-step denoising process. In this section, we examine the effects of applying C3 at various stages within this denoising process. We observe the changes in generated images by applying our method at six distinct points across a total of 50 steps. To quantify the degree of image change, we use LPIPS, a perceptual similarity metric, to compare the results at each stage with those generated by the proposed method. The LPIPS scores, averaged across 100 different images and random seeds, are shown in Figure~\ref{fig:step}-(top). Both the LPIPS scores and exemplar images show that when C3 is applied after the fifth step (Figure~\ref{fig:step}-(c)), the resulting images increasingly resemble the original, diverging from those generated with C3 applied continuously at each step. This analysis demonstrates that the impact of our method is most pronounced when applied in the early stages of the diffusion process, aligning with prior analyses on diffusion models that suggest structural content is primarily established in the earlier timesteps~\cite{yu2023freedomtrainingfreeenergyguidedconditional}.


\subsection{Types of Creativity}
\label{sec:exp_creativity_type}
We investigated which aspects of creativity are enhanced in images generated by the proposed method.
% For 50 images generated with C3 and 50 images from the original SDXL-Lightning model, we identified whether the creativity of each image corresponds to shape, texture, or color. 
This identification was performed using a multi-modal LLM (GPT 4o~\cite{achiam2023gpt}) to extract responses. The statistical findings, displayed in Figure~\ref{fig:type}, reveal that images generated by our method, depicted in vivid colors, achieve significantly higher values than those from the original model, shown in muted colors, highlighting an overall increase in creativity. Furthermore, we observe that different creative aspects are emphasized for each object type. For example, in the case of a chair, creativity is enhanced primarily in the shape aspect, garments in texture, and teddy bears in color. This suggests that our model effectively identifies and emphasizes suitable creative attributes for various objects, enhancing the generated images accordingly.


\begin{figure}[h!]
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  
         \includegraphics[width=0.9\columnwidth]{figure/creativity_type.pdf}
         \caption{
         Types of creativity classified by GPT 4o for Lightning (1-step) generations. Responses are multiple-choice, among `Shape', `Texture', and `Color'. 50 images are used for each method.
         }
         \label{fig:type}
  
\end{figure}


\subsection{Use Cases}
\noindent\textbf{Integration with ControlNet~\cite{zhang2023adding}.} To demonstrate the versatility of C3, we integrate it with ControlNet, a widely recognized plugin adapter. As shown in Figure~\ref{fig:ctrlnet_1}, this combination enables effortless generation of creative samples while adhering to input constraints. 

\begin{figure}[h!]
  \centering
         \includegraphics[width=\columnwidth]{figure/controlnet_app.pdf}
         \caption{Combining C3 with ControlNet on SDXL.}
         \label{fig:ctrlnet_1}  
\end{figure}

\noindent\textbf{Integration with SDXL Hyperparameters.}
We compare the results of our method with the readily available hyperparameters of the SDXL model, specifically in terms of classifier-free guidance (CFG)~\cite{ho2022classifierfreediffusionguidance} scale and negative prompts. CFG is a hyperparameter that regulates the blend between the outputs of the given prompt and the negative prompt. Higher CFG values are known to enhance text-image alignment. However, we have observed that, in some cases, there are only marginal improvements in creativity, even with large CFG values. As illustrated in Figure \ref{fig:cfg}, increasing the CFG from the default setting of 5 to 30, or using a negative prompt such as 'normal teddy bear', results in less significant changes in creativity. Conversely, our method enhances the default results without utilizing CFG or negative prompts. It is noteworthy that our method can also be employed alongside CFG and negative prompts, yielding more creative samples across all four settings.

% \begin{figure}[ht]
%   \centering
%   %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  
%          \includegraphics[width=\columnwidth]{figure/cfg.pdf}
%          \caption{
%          Comparisons between pre-defined Hyperparameter controls of SDXL and \textbf{C3}. \textbf{(Default)} CFG=5 / Negative prompt=``". \textbf{(CFG)} CFG=30. \textbf{(Neg)} Negative prompt=``normal teddy bear".
%          }
%          \label{fig:cfg}
  
% \end{figure}
\noindent \textbf{Extension to Alternative Prompts.} Our method is designed to function with textual descriptions that include \textit{``creative"}. To assess the versatility of our approach, we tested whether similar effects could be achieved using alternative templates beyond ``creative." In Figure~\ref{fig:template}, we constructed prompts using a total of four similar adjectives, $\{\textit{creative, rare, innovative, ingenious}\}$, and analyzed the outcomes when integrated with C3. We observed that across all templates, distinct and creative characteristics were expressed just as effectively as with ``creative." This suggests that C3 consistently enhances creativity across a range of creativity-associated prompts.

\begin{figure}[ht]
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  
         \includegraphics[width=0.75\columnwidth]{figure/template_change.pdf}
         \caption{Example outcomes using alternative prompts in place of 'creative.' 
         %Utilizing similar concepts still produces satisfactory results. 
         }
         \label{fig:template}
\end{figure}



% \begin{figure}[h]
%   \centering
%          \includegraphics[width=0.5\columnwidth]{figure_reb/kandinsky.pdf}
%          \caption{(Left) Block-wise amplified images on Kandinsky 3.0. (Right) Results of C3 applied on Down blocks of Kandinsky 3.0.}
%          \label{fig:kandinsky}  
% \end{figure}
\subsection{C3 on Non-SD Models}
 We applied C3 to Kandinsky 3.0 and HunYuan-DiT, in addition to SDXL variants. Kandinsky 3.0 is based on U-Net structure as SDXL, while HunYuan-DiT is based on stacked transformer structure. 
 The block-wise analysis for each model is provided in Appendix~\ref{sec:app_nonsd}. 
 % In Figure~\ref{fig:nonsd}, the results demonstrate the potential extension of our method to other text-to-image generative diffusion models with diverse architectures. However, specific model components such as normalization layers may influence its applicability. In particular, for transformer-based models with deeper architectures, a more detailed analysis is required to understand the impact of our method. 
 While Figure~\ref{fig:nonsd} opens the possibility of expanding C3 to non-SDXL-based models, the specific architecture and components of the model may affect the application of C3 to other models and more comprehensive analyses might be needed especially to understand transformer-based models, which we leave as future work. 



% \begin{figure}[h]
%   \centering
%          \includegraphics[width=0.8\columnwidth]{figure/nonsd.pdf}
%          \caption{Application of C3 on Kandinsky 3.0 and HunYuan-DiT models. }
%          \label{fig:nonsd}  
% \end{figure}
\vspace{-0.2cm}
% \noindent\textbf{Transformer-based Model.}
% In Figure~\ref{fig:dit}, we applied C3 on Hunyuan-DiT.
% %, consisting of 40 transformer blocks, and present results . 
% % In the right plot of Figure~\ref{fig:dit}, we present the blockwise LPIPS score between the original generation and the amplified generation (right) and the generated samples (left). 
% %In general, blocks 5-20 show the greatest variation when amplified. After blocks 20, we do not see significant variation even when maximally amplified. 
% Amplifying blocks 5–20 yields the most variation, while blocks beyond 20 show minimal change even at maximum amplification. Nevertheless, the impact of C3 on transformer-based models requires careful study, which we leave for future work.
%However, further detailed analyses are required to comprehensively understand the transformer models, including the role of each block, which we leave for future research. 

% \begin{figure}[h!]
%   \centering
%          \includegraphics[width=0.8\columnwidth]{figure_reb/dit2.pdf}
%          \caption{(Left) Images generated with amplified features for the ith transformer block of Hunyuan-DiT. (Right) Block-wise LPIPS score between the original image and the amplified image.}
%          \label{fig:dit}  
% \end{figure}
% \subsection{Failure Cases}
\subsection{Comparison with FreeU}
% \noindent\textbf{Comparison with FreeU}

Unlike FreeU~\cite{si2024freeu}, which enhances image fidelity by modifying low-frequency components in skip connections and boosts backbone features without frequency-based control—using uniform parameters $s$ and $b$ across layers—C3 specifically targets low-frequency backbone features in the down and middle blocks, applying layer-specific parameters. This distinction allows C3 to better steer creativity. As shown in Figure~\ref{fig:freeu}, FreeU produces less clean and creative results than C3, regardless of parameter values. Especially, when $b > 1$, noise persists regardless of $s$.


% C3 aims to enhance creativity via selectively amplifying feature representations. FreeU modifies low-frequency components in skip connections using uniform parameters $s$ and boosts backbone features without frequency-based control ($b$) across layers, resulting in limited adjustments. In contrast, C3 targets the low-frequency backbone (down and middle blocks) features and applies layer-specific parameters. This distinction enables C3 to better steer creativity. In Figure~\ref{fig:freeu}, FreeU yields less clean and creative results than C3, regardless of parameters. Especially, for $b > 1$, noise persists irrespective of $s$.


% C3 enhances creativity by selectively amplifying low-frequency backbone features with block-specific parameters, while FreeU~\cite{si2024freeu} attenuates low-frequency skip features ($s$) and boosts backbone features without frequency-based control ($b$), prioritizing fidelity. This distinction enables C3 to better steer creativity. In Figure~\ref{fig:freeu}, FreeU yields less clean and creative results than C3, regardless of parameters. Especially, for $b > 1$, noise persists irrespective of $s$.
% \begin{figure}[h!]
%   \centering
%          \includegraphics[width=\columnwidth]{figure/freeu-comparison-v2.pdf}
%          \vspace{-0.8cm}
%          \caption{Results with prompt  ``A creative chair'' in SDXL-Turbo.}
%          \label{fig:freeu}
  
% \end{figure}
